The Motivic Cohomology of Stiefel Varieties

The main result of this paper is a computation of the motivic cohomology of varieties of n \times m-matrices of of rank m, including both the ring structure and the action of the reduced power operations. The argument proceeds by a comparison of the general linear group-scheme with a Tate suspension of a space which is A1-equivalent to projective n - 1-space with a disjoint basepoint.

==> algebraicGeometryHeader.tex <==
\input{algebraHeader}

\newcommand{\spec}{\operatorname{Spec}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\Spec}{\spec}


\newcommand{\Sm}{\cat{Sm}}

\newcommand{\Gm}{\mathbb{G}_m}

\newcommand{\pt}{\text{\rm pt}}

\newcommand{\opensub}[1][{}]{\overset{#1}{\hookrightarrow}}
\newcommand{\clsub}[1][{}]{\overset{#1}{\rightarrowtail}}

\newcommand{\shom}{\mathcal{H}\!om}

\newcommand{\Nis}{\text{\it Nis}}

\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Cl}{\operatorname{Cl}}

\newcommand{\Div}{\operatorname{div}}
\renewcommand{\div}{\Div}
\newcommand{\val}{\operatorname{val}}

\newcommand{\et}{\text{\'et}}

\newcommand{\A}{\mathbb{A}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{\sh}[1]{\mathcal{#1}}
\newcommand{\dual}[1]{\check{#1}}

\newcommand{\G}{\mathbb{G}}
\newcommand{\lspan}[1]{\left<#1\right>}
